Summarizing Unstructured Logs in Online Services

Logs are one of the most valuable data sources for managing large-scale online services. After a failure is detected/diagnosed/predicted, operators still have to inspect the raw logs to gain a summarized view before take actions. However, manual or rule-based log summarization has become inefficient and ineffective. In this work, we propose LogSummary, an automatic, unsupervised end-to-end log summarization framework for online services. LogSummary obtains the summarized triples of important logs for a given log sequence. It integrates a novel information extraction method taking both semantic information and domain knowledge into consideration, with a new triple ranking approach using the global knowledge learned from all logs. Given the lack of a publicly-available gold standard for log summarization, we have manually labelled the summaries of four open-source log datasets and made them publicly available. The evaluation on these datasets as well as the case studies on real-world logs demonstrate that LogSummary produces a highly representative (average ROUGE F1 score of 0.741) summaries. We have packaged LogSummary into an open-source toolkit and hope that it can benefit for future NLP-powered summarization works.

==> arXiv_ICSE SEIP/abstract.tex <==
Logs are one of the most valuable data sources for managing large-scale online services. 
After a failure is detected/diagnosed/predicted, operators still have to inspect the raw logs to gain a summarized view before take actions.
However, manual or rule-based log summarization has become inefficient and ineffective.
In this work, we propose LogSummary, an automatic, unsupervised end-to-end log summarization framework for online services. 
LogSummary obtains the summarized triples of important logs for a given log sequence.
It integrates a novel information extraction method taking both semantic information and domain knowledge into consideration, with a new triple ranking approach using the global knowledge learned from all logs.
Given the lack of a publicly-available gold standard for log summarization, we have manually labelled the summaries of four open-source log datasets and made them publicly available.
The evaluation on these datasets as well as the case studies on real-world logs demonstrate that LogSummary produces a highly representative (average ROUGE F1 score of 0.741) summaries.
We have packaged LogSummary into an open-source toolkit and hope that it can benefit for future NLP-powered summarization works.






% Operators resort to reading the raw logs for troubleshooting.
% However, manually analyzing logs has become labor-intensive and time-consuming because of the complexity of the services.
% We propose LogSummary, a novel approach towards automatic summarization for real-time logs. 
% The goal of LogSummary is to provide a clear and valuable summary of logs, which takes both semantic information and domain knowledge into consideration. 
% LogSummary makes the system interpretable for operators to troubleshoot services by producing a highly compressed (average compression ratio of 3.1\%) and readable summaries (average ROUGE F1 score of 0.741) of the target log stream.
% Given the lack of a publicly-available gold standard for log summarization, we manually labelled a summary gold standard for four existing open-source log datasets and open-source them.
% The automated evaluation on four public production log datasets and case studies on real-world logs demonstrate that the generated summaries are highly relevant and representative of the semantics of the input logs.
% We present LogSummary to highlight the promise of NLP-powered summarization for logs, and discuss the challenges in the online log analysis scenario that must be overcome to realize this vision.
% We have packaged LogSummary into an open-source toolkit and hope that it can be used for future research.

==> arXiv_ICSE SEIP/background.tex <==

\textbf{Log Templates.}
%日志很重要
% Service logs play an important role in service management. 
Log parsing usually serves as the the first step towards automated log analysis.
%%当前的日志模板提取方法 
The most popular log parsing approach is automatic template extraction~\cite{zhu2019tools,drain,ft-tree,logparse}, which extract constant fields (templates) from logs. %, \textit{e.g.}, LogSig \cite{logsig}, FT-tree~\cite{ft-tree}, IPLoM \cite{iplom}, Drain \cite{drain}, Spell\cite{spell} and LogParse \cite{logparse} 
For example, ``Interface *, changed state to down'' is the template of the first and fifth logs in Fig.~\ref{fig:logs}, and traditional log parsing methods can extract templates from historical logs automatically. 
However, operators continuously conduct software/firmware upgrades on services to introduce new features, fix bugs, or improve performance. These upgrades usually generate new types of logs, and it is required to update templates online~\cite{kabinna2018examining}.
Therefore, we incorporate our previous work, LogParse~\cite{logparse}, to extract templates in this work.  
LogParse~\cite{logparse} is an unsupervised framework which contains a classifier to distinguish the template words and variables at runtime. 
It can extract and learn templates online without retraining its model.


% More specifically, Drain \cite{drain} applies a heuristics-based template extraction method. LogParse \cite{logparse} trains a classifier to distinguish the template words and variables.

% mbine templates.There are many c coategories of template extraction approaches~\cite{zhu2019tools}. 
% The first category is cluster-based methods, in which log template forms a natural pattern of a group of log messages. From this view, template extraction can be modeled as a clustering problem, such as LogSig \cite{logsig}.
% Next is frequent items mining. Log templates can be seen as a set of constant tokens that occur frequently in logs, such as FT-tree~\cite{ft-tree}. 
% Iterative partitioning is used in IPLoM~\cite{iplom}. 
% Some methods use heuristics to extract templates. As opposed to general text data, log messages have some unique characteristics. 
% Consequently, works such as Drain \cite{drain} propose heuristics-based template extraction methods. 
% The final category is longest common subsequence. For example, Spell \cite{spell} uses the longest common subsequence algorithm to parse logs in a stream. 




% \subsection{Online Representation}\label{sec:measuerments-oov}
\textbf{Word Embedding for Logs.} 
Logs are designed to facilitate user readability. 
Consequently, the constant parts of logs are defined in human readable manner by developers. 
Many methods (\textit{e.g.,} word2vec~\cite{mikolov2013exploiting}) thus use natural language process (NLP) methods to represent words. 
However, these methods cannot represent domain-specific words accurately. 
For example, ``down'' and ``up'' in Fig.~\ref{fig:logs} are antonyms but they have similar contexts.
Besides, system upgrades usually generate new types of logs with unseen words~\cite{log2vec} (\textit{e.g.,} ``Vlan-interface'' in Figure~\ref{fig:logs}), which pose a challenge for generating distributed representations of words in logs.
% The current word embedding methods cannot embed these unseen words because they are usually trained offline based on the vocabulary of historical logs, which cannot be updated at runtime.
% For example, Fig.~\ref{fig:measure_oov_word} shows percentages of new words as the percentage of training data increases from 10\% to 90\%.
%We observe a large percentage of new words when trained on a smaller sample of the logs, which show that it's essential to handle new words when analyzing logs. %, specially when building distributed representations online which are required for the final output of downstream tasks.
For this reason, we adopt our previous work, Log2Vec~\cite{log2vec}, to represent the words of logs.
Log2Vec combines a log-specific word embedding method to accurately extract the semantic information of logs, with an out of vocabulary (OOV) word processor to embed unseen words into distributed representation at runtime.


% %%不同数据集下的OOV单词统计
% \begin{figure}
%       \begin{minipage}[h]{1.0\linewidth}
%       \centering
%       \includegraphics[width =8.6 cm]{./figures/oov-word-measure.pdf}\\
%       \end{minipage}
      
%       \caption{Measurements of new words.}\label{fig:measure_oov_word}
%     %   \vspace{-2 mm}
% \end{figure}

% %%不同数据集下的含OOV的日志统计
% \begin{figure}
%       \begin{minipage}[h]{1.0\linewidth}
%       \centering
%       \includegraphics[width = 8.6 cm]{figures/oov-log-measure.pdf}\\
%       \end{minipage}
%     %   \vspace{-1 mm}
%       \caption{Measurements of logs with new words.}\label{fig:measure_oov_log}
%     \vspace{-1.5 mm} 
% \end{figure} 

% \textbf{Text Summarization.} Lots of previous work in NLP domain focuses on text summarization generates summaries from input documents while keeping salient information. It is an important task in NLP domain and can be applied to several real-world applications. 
% There are two main text summarization techniques: extractive and abstractive. Extractive summarization generates summary by selecting salient sentences or phrases from the source text, while abstractive methods paraphrase and restructure sentences to compose the summary. Many popular extractive summarization techniques do not require example summaries and instead consider summarization as a sentence-selection (e.g, TextRank\cite{textrank}) or keyword-selection (e.g, LDA\cite{Ramage2009Labeled}) problem. Sentences may be selected based on scores computed from the presence of topic-words or word-frequencies \cite{nenkova2005impact}. Gaetano Rossiello \textit{et al.}~\cite{rossiello2017centroid} extends this approach by mapping sentences to their representation using word2vec embeddings rather than using TF-IDF weights. While abstractive summarization involves paraphrasing the context-aware sentences after understanding the language \cite{paulus2017deep,nallapati2016abstractive}. Abstractive techniques generally requires large-scale data (documents and corresponding summaries) for training the models, for example news titles can be considered as summaries and the articles can be considered as the document. However, logs do not have the corresponding summaries for training.
% The aforementioned works deal with properly written regular text and are not directly applicable to our domain. In contrast, LogSummary focuses on logs to extract domain-sepcific information and perform log summarization.
% Short-text summarization or compression has been tackled in the NLP field facing similar challenges to the ones we face with logs. Logs are pieces of short text that come in a temporal stream of data, which can also be found in other scenarios. In the field of NLP, short text analysis and mining has become more and more important with the advent of social media. Specifically for cases such as Twitter or Sina Weibo, which are an analogous scenario where a constant stream of short texts are generated.
% Short texts present different challenges from documents text corpus. Their representation becomes more challenging given the sparsity that it imposes if the usual bag of words and weighted representations are used. Additionally, there is less syntactic information to learn from if texts are short. 
% Common approaches such as latent Dirichlet allocation (LDA) \cite{Blei2003Latent} do not perform well on short text because of its inherent short length and therefore its sparseness. Considering such challenge, \cite{jipeng2019shorttext:survey} presents a survey on short text topic modeling techniques applications and performance. They divide these methods into three categories depending on their approach, these being Dirichlet multinomial mixture, global word co-occurrences, and self-aggregation. Particularly, the self-aggregation approach solves the sparseness problem in short texts by combining short texts into longer ones as pseudo-documents before applying topic modeling. LogSummary, takes an approach similar to self-aggregation, while using more fine-grained semantic pieces obtained from LogIE from each of the logs within the target log stream.


\textbf{Information Extraction.} Information extraction retrieves relational triples from unstructured text. This is usually done in the form of triples for binary relations, relating two arguments by a predicate or relation for each relation in a given sentence, \textit{i.e.} $(argument_{1}, relation_{1,2},argument_{2})$ \cite{Banko2008OpenIE}. Traditional information extraction approaches rely on predefining a limited set of target relations and hand-crafted patterns. For this they would adapt Named Entity Recognizers and dependency parsers to target a specific domain. These approaches would then require manual effort to be repurposed and applied to a different domain. In order to address the challenge of scalability for performing web information extraction, Banko \textit{et al}. \cite{Banko2008OpenIE} introduced Open Information Extraction (OpenIE). They presented a new information extraction paradigm that would allow to extract relations without defining the number or type of relations in advance.





% Therefore, we propose LogSummary, an automatic log summarization takes both semantic information and domain knowledge into consideration. The output of LogSummary are ranked summaries ( triples with ``entities'',  ``events'' and ``relation'' of them).
% We focus here on summarizing logs over a user-provided time period.



==> arXiv_ICSE SEIP/case-study.tex <==


To further evaluate the performance of LogIE, we did a case study on real-world logs, which are generated by switches deployed in a top cloud service provider. In this part, we selected and labelled one million switch logs in the same manner we did for the public datasets as described in Section \ref{sec:gt-logie}. Here results are consistent with the experiments on the public log datasets. Likewise, given that the proportion of free text is higher within this logs dataset, a complex OpenIE approach can also generate comparably accurate triples. Nonetheless, both LogIE approaches outperform all of the baselines at a throughput that is over 200 times higher. %Please note that while we open-source our produced log OpenIE triples gold reference dataset based on public logs, we do not do so with the logs from this case study.
For this real-world dataset, LogIE achieves F1 of 0.831, where other OpenIE methods get average F1 of 0.414.

Besides, we conducted a case study of LogSummary on switch logs to visualize its intermediate steps and showcase its results.
As shown in Figure~\ref{fig:case-study-logs}, we randomly selected 300 logs from real-world switch logs, applied LogIE to extract triples, and generated a summary with LogSummary. The corresponding weighted triple graph from TextRank is shown in Figure~\ref{fig:case-graph}.
This summarization result was confirmed by operators and prove that LogSummary is useful.

==> arXiv_ICSE SEIP/challenge.tex <==





% In this section, we first an overview of LogSummary. Next, we describe its design and implementation of its each parts.


\begin{figure}
      \begin{minipage}[h]{1.0\linewidth}
      \centering
      \includegraphics[width = 8.5 cm]{./figures/framework.pdf}\\
      \end{minipage}
%      \vspace{-1 mm}
       \caption{Framework of LogSummary}\label{fig:logsummary}
      \vspace{-1 mm}
\end{figure} 

\begin{figure}
      \begin{minipage}[h]{1.0\linewidth}
      \centering
      \includegraphics[width = 8.5 cm]{./figures/LogIE_diagram.pdf}\\
      \end{minipage}
    %   \vspace{-1 mm}
       \caption{Detailed workflow of the LogIE in LogSummary (Fig.~\ref{fig:logsummary}).}\label{fig:logie}
      \vspace{-1 mm}
\end{figure} 



The requirement to read and understand logs quickly in online services motivates the design and implementation of LogSummary. 
LogSummary is an automatic log summarization approach which takes both semantic information and domain knowledge into consideration. 
% The output of LogSummary are ranked summaries.

\subsection{Design Challenges}\label{sec:detail-challenge}
Log data is an important data source recording system states and significant events at runtime. 
It is thus intuitive for operators to observe system status and inspect potential anomalous events using logs.
A log is usually printed by logging statements (\eg printf(), logger.info()) in the source code, which are predefined by developers. Typically, the predefined part of a log is human readable. 
% Take Fig.~\ref{fig:logs} as a example, in the first log message, ``ae3'' is a $variable$ word, whereas the rest, \textit{i.e.}, ``Interface ..., changed state to down'', is the $constant$ field. 
Therefore, solving log summarization problems using NLP tools seems promising. 
However, directly applying existing NLP approaches for log summarization faces several challenges as follows.
% does not work. Operators still have to read raw logs and extract valuable information by themselves in practice. 
% In designing LogSummary, we need to solve several challenges.




\noindent\textbf{Domain-specific symbols and grammar.}
Logs contain many domain-specific symbols, and their grammer may significantly differ from normal sentences. 
Existing NLP tools, which are typically designed for normal sentences, cannot get accurate summaries for them. 
% We need to preprocess them by using domain knowledge and automatically extracted templates.
For example, entity-value pairs are valuable and structured information that should be extracted from unstructured logs.
However, existing NLP tools cannot extract them directly,
% They should be preprocessed before utilize NLP tools.
because they may be separated by an equal ``='' or a colon ``:'' symbol. 
Besides, some entity-value pairs are hidden in word combination. 
For instance, when NLP tools process the first log in  Fig. \ref{fig:logs},  it may treat ``Interface ae3'' as a whole, while ``ae3'' is a value for the entity of ``Interface''.


\noindent\textbf{High summarization efficiency requirement.}
After a failure is detected or predicted, operator hope to quickly obtain the summary of a collection of logs in some period (\eg one hour before a detected failure) to figure out what happens on the online service.
However, the online service can generate a large number of logs in this period.
% There are huge amount of logs. 
% Specifically, tens of millions of log messages are generated by online systems everyday. 
For example, one program execution in the HDFS system generates 288,775 logs per hour~\cite{deeplog}.
% When operators read logs, our system should provide summaries immediately.
% However, processing each log is time consuming. 
On the other hand, existing NLP methods typically get the summarized triples one sentence (log) by one sentence (log), and their efficiency cannot satisfy the requirement of operators (see Table~\ref{table:logie-speed} for more details).




\noindent\textbf{Obtaining the summarized triples of important logs.}
Typically, logs are generated in the order of program executing, and they contain redundancy and repetition.
When operators inspect a collection of logs triggered by a failure detection or prediction, they want to obtain the triples of those \emph{important} logs first.
However, existing NLP approaches usually generate summaries according to the order of sentences (logs) in the original text (log sequence).
In Fig. \ref{fig:case-study-logs}, for example, an state-of-the-art NLP method generates summaries by compressing original logs, instead of generating the triples of the expected important logs.
Consequently, these approaches cannot satisfy the expectation of operators.

% Operators prefer to choose and read important events first. 
% NLP tools usually generate summaries based on the order of original text, which conflict with the expectations of operators. 



% Logs are generated in the order of program executing, text summarization methods also generate summaries based on the order of original text, which conflict with the expectations of operators. Operators prefer to choose and read important events first, however traditional methods cannot rank summaries based domain-specific meaning.

\noindent\subsection{Overview of LogSummary}\label{sec:overview}

In this section, we design LogSummary (as shown in Fig.~\ref{fig:logsummary}) to summarize logs in online services and help operators to read/understand logs faster. LogSummary have two parts, offline training and online summarization.


During offline training, LogSummary applies unsupervised template extraction methods \cite{zhu2019tools} to get templates from historical logs. These templates are used by LogIE in the online stage for matching and processing logs.%Templates handle the challenge that logs contains domain-specific text.
%
Since it's nearly impractical to rank arbitrary summaries, LogSummary applies Log2Vec \cite{log2vec} to learn the semantics of logs and train word embeddings. Log2Vec not only learns domain-specific semantics from offline logs, but also generates a new embedding for unseen (OOV) words at runtime, which are common in new generated logs in online systems. Then, LogSummary applies the trained embeddings to rank summaries online.



In the online stage, we design LogIE (describe in Section \ref{sec:logie})  a mechanism to generate triples for given logs. The inputs of LogIE are real-time logs and templates. LogSummary updates new templates automatically by using LogParse \cite{logparse}. LogIE outputs summaries of logs. LogIE solves the challenge that logs contain domain-specific text. Besides, LogIE saves mapping caches between triples and templates, which speeds up log processing and solves the processing speed challenge imposed by the huge amount of logs.
%
After LogIE, LogSummary ranks triples by adopting TextRank, which meets the requirements of operators reading important summaries first rather than following the program execution logs order.









==> arXiv_ICSE SEIP/conclusion.tex <==
%%
Logs play an important role in service maintenance. 
Operators still have to conduct log summarization before take actions in a manual or rule-based manner, even though many methods have been proposed for automatic log detection/diagnosis/prediction.
% reading the log stream for troubleshooting.
In this paper, we propose LogSummary, a framework towards automatic summarization for large-scale online services. 
LogSummary combines LogIE, which accurately and efficiently obtains information extraction triples from logs, and a simple yet effective triple ranking method, which utilizes the global knowledge learned from all historical logs.
We perform extensive evaluation experiments to demonstrate LogSummary's performance in summarizing logs. 
Moreover, we have open-sourced LogSummary and the manually labelled gold standard references, hoping that they can benefit for future research works. 




% Logs play an important role in service maintenance. 
% Log representation is the first step of automated log analysis. 
% However, the current log representation methods cannot represent domain-specific semantic information of logs and cannot handle out-of-vocabulary words at runtime. 
% We propose a semantic-aware representation framework, \name{}, to improve the performance of online log analysis. 
% We present a measurement on OOV words and evaluate the performance of OOV word processor in \name{}.
% In addition, we apply \name{} to two popular log-based service management tasks, including log classification and anomaly detection, both demonstrating that \name{} can extract the crucial features of logs and significantly improve the performance of them.
% Since \name{} is able to assign/generate a ``soft'' representation for any given log, we will achieve other novel log analysis applications by adopting \name{}.
% Traditional log representation methods limit many log analysis applications, which require to have a representation for any log.
% Log2Vec is able to assign a ``soft'' representation to every log at runtime, in order to avoid false alarms induced by new types of logs, we will improve log-based service management tasks (\textit{e.g.}, failure prediction, root cause analysis) by adopting Log2Vec in the future.





==> arXiv_ICSE SEIP/design.tex <==


\subsection{LogIE}\label{sec:logie}
In order to accurately and efficiently extract valuable information from logs, we propose LogIE (Log Information Extraction). 
%
LogIE performs open information extraction on logs, extracting triples relating entities and arguments through a relation or predicate. To achieve this, it combines both Rule Extraction (RE) and OpenIE to extract the triples. 
In order to make the process fast and efficient, LogIE adopts templates to improve and speed up information extraction of logs.
Note that, templates are extracted by existing approaches \cite{zhu2019tools,logparse} automatically.
LogIE learns triples from the log templates, so template matching can be used to produce the LogIE triples output.
% In this way, LogIE extracts valuable information from logs in a structured manner to aid downstream tasks (\textit{e.g.,} log stream summarization. 
LogIE is a framework composed of four main components, which we describe and explain how they work using the simple example in Fig. \ref{fig:template}.


\begin{figure}
    $\underbrace{\text{Link bandwidth lost totally is resumed.}}_{\text{Free Text}}\ \underbrace{\text{( Reason = }\overbrace{\text{*}}^{\text{VAR1}} \ )}_{\text{Structured Text}}$
    \caption{Log template example.}
    \label{fig:template}
\end{figure}
% We can keep this as a figure so we can have a caption and reference it more easily or change it to an "align*" and lose the caption.












\subsubsection{Matching $\And$ Processing}
Matching and Processing are the overarching components of LogIE supported by the RE and the OpenIE components that perform the triple extraction. As shown in Fig. \ref{fig:logie}, LogIE takes both raw logs and templates as its input. LogIE performs template matching on the input rawlogs. Using Fig. \ref{fig:template} as an example, if a log is matched with this template, LogIE retrieves the previously extracted triples for this given log-type and substitute the variables present in the triples by their actual value obtained from the raw log. These variables are usually identifiers, values or service addresses \cite{pi2019semantic}. Therefore once a log is received, if a template is matched by the matching component, it will directly be processed by the Processing component and output its LogIE triples. This way LogIE is able to effectively and efficiently yield OpenIE triples in an online manner. 
Since the goal of LogIE is to get a structured information from logs, we treat all these cases equally by substituting them by a dummy token to be considered an entity or part of an argument \textit{e.g.,} "VARX", where X is the ordinal of the variable within the template.
In the case that the log is not matched to any template, a new template needs to be extracted\cite{drain,logparse}. Since LogIE is meant to be run online, it requires a template extraction and matching method that can be incrementally updated online. For this reason, we incorporate LogParse into the Matching component. The new template is then split into subparts as shown in Fig. \ref{fig:template}, based on rules predefined accordingly to the source services log. These subparts are then handled by the RE and OpenIE components to extract a new set of triples from it. The RE component would handle the structured parts, while the OpenIE one handles the free text parts. The output triples are then stored and passed to the Processing component to produce the final LogIE triples output. 


\begin{algorithm}[t] %算法开始 
\caption{Log Summarization} %算法的题目 
\label{alg:summarization} %算法的标签 
\begin{algorithmic}[1] %此处的[1]控制一下算法中的每句前面都有标号 
\REQUIRE A semantic information triple set  $ST$, a domain knowledge triple set $DT$,  the number of triple candidates $k$  and word embedding set $WE$ %
%输入条件(此处的REQUIRE默认关键字为Require，在上面已自定义为Input) 
\ENSURE Ranked summaries $S$  %输出结果(此处的ENSURE默认关键字为Ensure在上面已自定义为Output) 

%first-level%
\STATE Create a triple vector set $TV$
\FOR{each triples $st$ of $ST$} 
\STATE Create a temporary empty triple vector $tv$
\STATE Let a integer variable $len$ record the number of words in $st$
\FOR{each word $w$ of $st$} 
\STATE Find the corresponding word vector $wv$ for $w$ in $WE$
\STATE Plus the current word vector $wv$ to the temporary triple vector $tv$
\ENDFOR 
\STATE Get the average vector $av$ by dividing $tv$ by $len$ and regard $av$ as the triple vector $st$
\STATE Append the triple vector $av$ to $TV$
\ENDFOR 
\STATE Init a matrix of transition probability $M$ by calculating cosine similarity between all $tv$ pairs in $TV$
\STATE Convert $M$ to a weighted graph $G=(V,E)$. 
\STATE Get the triple scores $TS$ by applying Formula~\ref{equation} to $G$
\STATE Sort the triples in reverse order by scores in $TS$, and the top $k$ triples as the final summaries $S$.
% \STATE Sort the triples in reverse order by scores in $TS$, and the top $k$ triples as the first-level summaries $S$.

% %second-level%
% \STATE Create a list $S_2$ for second-level summary 
% \FOR{each $st$ of $S_1$} 
% \STATE Find the corresponding domain knowledge vector $dt$ for $st$ in $DT$
% \STATE Append $dt$ to $S_2$
% \ENDFOR 

%return%
\RETURN $S$
\end{algorithmic} 
\end{algorithm}


% \begin{algorithm}[t] %算法开始 
% \caption{Log Summarization} %算法的题目 
% \label{alg:summarization} %算法的标签 
% \begin{algorithmic}[1] %此处的[1]控制一下算法中的每句前面都有标号 
% \REQUIRE A semantic information triple set  $ST$, a domain knowledge triple set $DT$,  the number of triple candidates $k$  and a Log2Vec word embedding set $WE$%输入条件(此处的REQUIRE默认关键字为Require，在上面已自定义为Input) 
% \ENSURE First-level summary $S_1$ and second-level summary $S_2$ %输出结果(此处的ENSURE默认关键字为Ensure在上面已自定义为Output) 

% %first-level%
% \STATE Create a triple vector set $TV$
% \FOR{each triples $st$ of $ST$} 
% \STATE Create a temporary empty triple vector $tv$
% \STATE Let a integer variable $len$ record the number of words in $st$
% \FOR{each word $w$ of $st$} 
% \STATE Find the corresponding word vector $wv$ for $w$ in $WE$
% \STATE Plus the current word vector $wv$ to the temporary triple vector $tv$
% \ENDFOR 
% \STATE Get the average vector $av$ by dividing $tv$ by $len$ and regard $av$ as the triple vector $st$
% \STATE Append the triple vector $av$ to $TV$
% \ENDFOR 
% \STATE Init a matrix of transition probability $M$ by calculating cosine similarity between all $tv$ pairs in $TV$
% \STATE Convert $M$ to a weighted graph $G=(V,E)$. 
% \STATE Get the triple scores $TS$ by applying Formula~\ref{equation} to $G$
% \STATE Sort the triples in reverse order by scores in $TS$, and the top $k$ triples as the first-level summary $S_1$.

% %second-level%
% \STATE Create a list $S_2$ for second-level summary 
% \FOR{each $st$ of $S_1$} 
% \STATE Find the corresponding domain knowledge vector $dt$ for $st$ in $DT$
% \STATE Append $dt$ to $S_2$
% \ENDFOR 

% %return%
% \RETURN $S_1$ and $S_2$
% \end{algorithmic} 
% \end{algorithm}



\subsubsection{RE for Rule Triples}\label{sec:rule-triples}
The purpose of the RE component is to make the most out of the structure present in logs, namely the structured text part from the example in Fig. \ref{fig:template}.
According to our observation, there are some rules for systems to print logs. Therefore it becomes easier to define rules to extract part of the information present precisely. For example, in our implementation, we use three different rules, where all three cover different ways of representing entity-value pairs. For these cases, entity-value pairs are usually separated by an equals “=” or a colon ``:" symbol. 
Another common case, is formatting such information in the same way command line arguments are specified in a command line interface program. 
% For all these cases, following the IE triple format, we use "is" as a predicate relating the entity to its instance or value e.g. ("Reason", "is", "VAR1"). 
% \textcolor{red}{For the case when the command line arguments format specifies a flag to be set, we also use "is" as predicate and define the second argument as "set". }
The outputs of the RE component of LogIE could be used to provide further details of the log stream in a readable structured manner, or store structured information (entity-value pairs) for further data mining.
Besides, the RE component processes unstructured logs by first extracting triples from the non-free text parts of the logs before the OpenIE component processes their remaining free text parts.

\subsubsection{OpenIE for Semantic Triples}\label{sec:semantic-triples}
Operators pay attention to ``entities'',  ``events'' and the ``relation'' between them when they read logs which making these the most important pieces of information to be considered for log summarization.
OpenIE \cite{Banko2008OpenIE} is usually used to extract relational triples, which is exactly what the operators need, since they are both structured in a human readable way~\cite{ApplicationsMausam2016OpenIE}, and a reduced version of the original logs.% that will be combined with the output of the rules extraction component. 
After rule triples were extracted using templates, the remainder free text is passed on to OpenIE component. 
There has been substantial progress on OpenIE approaches since it was proposed by Banko et al. \cite{Banko2008OpenIE}. 
These methods take free text as input and yield OpenIE triples as the output, formed by two arguments related by a predicate e.g. (``Link bandwidth", ``is", ``resumed"). OpenIE methods achieve their objective by leveraging the underlying semantic structure of the sentences for a given language enabling them to find the arguments present and the predicates that relate them. We therefore leverage existing OpenIE approaches in our implementation to fulfill the OpenIE component requirement of the LogIE framework. 
Since LogIE is a framework, none of its components, including OpenIE, are tied to any implementation in particular. 
Besides, many short logs do not have whole three element of triples, \eg, do not contain entity, OpenIE can also generate ``triples'' with less than three elements.
The output of the OpenIE component are the semantic triples, LogSummary will rank them and generate the summary later.
As you will see in our evaluation in Section \ref{sec:evaluation}, we incorporate the main OpenIE methods from the literature into our work as both baselines for LogIE and as part of the LogIE framework for evaluation.


\subsection{Ranking Summaries}\label{sec:summarization}
As aforementioned, logs, which record the status of services in real-time, usually suffer from redundancy and repetition. Traditionally, operators need to read raw logs and extract valuable information manually. 
However, it‘s labor-intensive and time-consuming.
% \textcolor{red}{
The goal of the LogSummary is to help operators to read/understand logs faster. 
After the LogIE stage, we obtain triples, the minimum units of semantic information within logs. 
In this section, we introduce a mechanism to rank the triples based on their informativeness. 
% they usually use knowledge drawn from entire logs to make local ranking decisions.
Operators generally hope to find out the importance of each triple by measuring the connection between each triple and other triples. For a set of logs, most algorithms ignore the semantics and other elements of its words, and simply treat a triple as a collection of words. And each word appears independently and does not depend on each other. However, in log analysis domain, different word combinations have different meanings. 
Operators usually use knowledge drawn from entire logs to make local ranking decisions.
Therefore, we integrate the information of the global corpus into the sorting algorithm in the form of word vectors, and through the combination of the sorting algorithm and word vectors, iteratively score sentences and sort them according to the score.
% }

\subsubsection{Triple Representation}\label{sec:triple-representation}

Firstly, we propose a method to represent triples with domain-specific semantic.
% Our goal is to assign an accurate sensible embedding for triples in the logs at runtime, which base on domain specific semantic learned from offline and is able to handle any triples.
% Current word embedding methods in NLP domain usually fail to capture the precise meanings of many words in logs, because some pairs of opposites may have similar contexts. 
% For example, ``down'' and ``up'' in Fig.~\ref{fig:logs} are antonyms but they have similar contexts. Additionally, as per the observations mentioned above, previously unseen words pose a challenge for building distributed representations during runtime.To resolve these problems, we adopt Log2Vec~\cite{log2vec}, a semantic-aware word representation method for online logs.
Log2Vec~\cite{log2vec} enables generalization to domain-specific words, which is achieved by integrating the embedding of lexical and relation features into a low-dimensional Euclidean space. 
By training a model over the existing vocabulary, Log2Vec~\cite{log2vec} can later use that model to predict the embedding of any words, even previously unseen words at runtime. 
Therefore, we apply the technique in Log2Vec to represent triples generated from logs.
% In order to calculate the ``similarity'' among them, we need to generate vectors from any triple. 
Leveraging its previous components, we converts any word in the triples into a word embedding vector and generates the triple's vector, which is the weighted average of its word vectors.



\subsubsection{Ranking Triples}\label{sec:triple-rank}
% In service management, operators usually read logs to find which events occur, and then, they find which variables (\textit{e.g.}, models, interfaces) are related to these events. 
% Inspired by this process, we propose a two-level summarization approach based on LogIE triples.
% In the first level summaries, we show valuable information to describe the events. In the second level summaries, we show the structured data for operators to query and further troubleshooting.

%介绍operators的需求场景->引出textrank

In this section, we propose a method to rank log summaries. %, which combines LogIE triples and TextRank\cite{textrank}. 
Its workflow is shown in Algorithm~\ref{alg:summarization}. 
%
Firstly, we build a graph associated with the logs, where the graph vertices are representative for the units to be ranked. For the application of triple extraction, the goal is to rank entire semantic triples, and therefore a vertex is added to the graph for each triple in logs. 
Same as sentence extraction, we define a relation that determines a connection between two triples if there is a ``similarity'' relation between them, where the ``similarity'' is measured as the cosine similarity~\cite{gravano2003text} of two triples. Note that, other similarity measures (\textit{e.g.,} Euclidean distance~\cite{danielsson1980euclidean}) are also possible.
Such a relation between two triples can be seen as a process of ``recommendation'': given a triple that addresses certain concepts in logs, it is ``recommended'' to refer to other triples in the logs that address similar concepts. 
Therefore a similarity link is drawn between any two triples.

\begin{figure}
      \begin{minipage}[h]{1.0\linewidth}
      \centering
      \includegraphics[width = 8 cm]{figures/triple_networks.pdf}\\
      \end{minipage}
%       \vspace{-1 mm}

       \caption{Weighted graph of case study on real-world switch logs.}\label{fig:case-graph}
    % \vspace{-2 mm} 
\end{figure} 

Unlike the unweighted graphs in PageRank~\cite{page1999pagerank}, we need to build weighted graphs.
The resulting graph is highly connected, with a weight associated with each edge, indicating the strength of connections established between various triple pairs in logs. The logs are therefore represented as a weighted graph (Fig.~\ref{fig:case-graph} shows a weighted graph for the case study in Section \ref{sec:experiment-summary}).
Formally, let $G=(V, E)$ be a directed graph with the set of vertices $V$ and set of edges $E$, where $E$ is a subset of $V * V$. For a given vertex $V_i$, let $In(V_i)$ be the set of vertices that point to it and let $Out(V_i)$ be the set of vertices that vertex $V_i$ points to.
Then, we adopt the formula in TextRank~\cite{textrank}, which is for graph-based ranking that takes into account edge weights when computing the score associated with a vertex in the graph. Textrank's formula is defined to integrate vertex weights.


\begin{equation}
\label{equation}
WS(V_i) = (1-d) + d*\sum_{V_j\in In_{V_i}}\frac{w_{ji}}{\sum_{V_j\in In_{V_i}}w_{jk}} WS(V_j)
\end{equation}
where $d$ is a damping factor that can be set between 0 and 1.

% \begin{figure}
%       \begin{minipage}[h]{1.0\linewidth}
%       \centering
%       \includegraphics[width = 7.5 cm]{figures/triple_networks.pdf}\\
%       \end{minipage}
% %       \vspace{-1 mm}
%       \caption{Example of a triple graph}\label{fig:triple-graph}
% %     \vspace{-4 mm} 
% \end{figure} 

After the triple-based TextRank~\cite{textrank} is run on the graph, semantic triples are sorted in reverse order of their score.%, and the top-ranked triples are selected for inclusion in the first-level log summaries.
% For first-level summaries, if two triples have the same prefix, we merge the matching parts. In Fig.~\ref{fig:logs}, for example, Algorithm~\ref{alg:summarization} generates ``(Interface, changed to, down)'' and ``(Interface, changed to, up)'', we merge the matching parts and get ``Interface changed to down up"". 
Note that, although the summaries of LogSummary are highly compressed, it have different goal with other log compression applications (\textit{e.g.,} LogZip\cite{logzip}). 
Other log compression applications aim to store logs while our summary are more readable for operators.

% \textcolor{orange}{For the second-level summaries, we need to show the triples for domain knowledge which are structured data for operators to query.
% The triples for domain knowledge have been generated in LogIE phase. In summarization phase, we select the triples (with ``is'' relation) that are related to the first-level summaries. In Fig.~\ref{fig:logs}, for example,  we show ``Interface changed to down up'' in the first level summaries, and then, show the detailed information for ``Interface'', \textit{i.e.,} ``Interface : ae3''.}












==> arXiv_ICSE SEIP/discussion.tex <==

The LogSummary framework leverages each of its components to automatically produce accurate summaries. However, its pipeline nature makes each component dependant on the quality of the output from the previous ones. Therefore, the quality of the templates may affect the triples extracted by LogIE, which in turn affects the representations built by Log2Vec \cite{log2vec} which are used by TextRank \cite{textrank} to produce the final summary of LogSummary. Nonetheless, each of the components provides significant benefits over their baselines. LogIE produces triples at over 200 times the throughput of plain OpenIE methods, which serve as the intermediate result that LogSummary leverages to achieve $\approx$4.6 times the recall of TextRank \cite{textrank}, which is the best performing baseline.
Both LogSummary and LogIE can serve further downstream purposes, which we consider for future work. The triples output of LogIE could aid the creation of knowledge graphs applied to perform automatic root cause analysis. Additionally they could serve as the intermediate representation before other log analysis tasks. LogSummary could produce the summary of anomalous logs for troubleshooting.
Further, we consider five log datasets as part of the evaluation from online system services. Our approaches outperform their baselines in all of them, which shows the generalizability of LogSummary.


% brainstorming
% We can discuss the subjectivity of the summarization evaluation and how we reduce it with the gold standard

% Analysis: the difference between logIE and OpenIE, and why we run fast. 


% The importance of the quality of the templates given that its a pipeline method for LogIE. Similar points for LogSummary.

% We could explain that we use the gold standard as input and it performs better than the online one but this is a novel approach and we pave the way for future improvement

% Discuss somehow about the novelty of logsummary and its pros/(cons) in its application

%Future works: We could apply LogIE to build knowledge graph for root cause analysis. Structured triples are intermediate representations in other log analysis tasks (\textit{e.g.,} log-based anomaly detection).  We can use LogSummary to do alarm compression.

% One limitation of LogSummary is that it is a pipeline framework, which consists of many modules. If previous modules perform bad, the output of LogSummary may be bad as well. For example, the accuracy of template extraction is essential to LogSummary.




==> arXiv_ICSE SEIP/evaluation.tex <==
In this section, we report all experiments conducted to evaluate the effectiveness of the proposed LogSummary.
We evaluate LogSummary from two aspects. 
Firstly, we evaluate the accuracy of LogIE on information extraction and compare it with common information extraction approaches. 
Next, we evaluate the accuracy of ranked summaries on the gold references and compare it with the baselines. 


\subsection{Experimental Setting}\label{sec:setting}

\subsubsection{Datasets}\label{sec:datasets}
We conduct experiments over four public log datasets from several services: BGL logs~\cite{Xu2009Detecting}, HDFS logs~\cite{deeplog}, HPC logs~\cite{lin2016log}, and Proxifier logs\cite{logzip}.

Since the lack of a publicly-available summary gold standard hinders the automatic evaluation, we manually labelled the above public log datasets and make them available\footnote{https://github.com/LogSummary/ICSE2021/tree/main/data}. 
In this paper, we provide two kinds of gold standard datasets. For information extraction, we labelled all templates for all logs (\cite{zhu2019tools} only label templates for 2000 logs per dataset) and labelled OpenIE triples leveraging semantic information and domain knowledge. 
To evaluate log summarization, we chose 100 groups of 20 contiguous logs per dataset and generated their summaries manually.

% Besides, to further evaluate the performance of LogSummary, we also show case studies on real-world logs, where logs are generated by switches deployed in a top cloud service provider.
The detailed information of above datasets are listed in Table~\ref{tab:datasets}. 


\begin{table}[!ht] %%表格在中间线两侧
\centering
\caption{Detail of the service log datasets.}\label{tab:datasets}
\renewcommand\tabcolsep{2.75 pt} % 调整表格列间的宽度
\begin{tabular}{ccc}%表示创建一个4列的表格环境，其中 l靠左，c居中。
\toprule
Datasets&Description&\# of logs\\ %表格内换行用\\
\midrule
BGL&Blue Gene/L supercomputer log& 4,747,963\\ %32.00 MB 
HDFS&Hadoop distributed file system log& 11,175,629 \\%48.61 MB
HPC&High performance cluster log& 433,489 \\%9.95 MB
% Spark&Spark job log& 33,236,604\\ %1.47 GB
Proxifier&Proxifier software log& 21,329 \\%48.61 MB
% Zookeeper&ZooKeeper service log& 74,380 \\%48.61 MB

% Switch&Network switch log&1,000,000 \\%48.61 MB
%BGL&Blue Gene/L supercomputer log&4,747,963 \\%48.61 MB
\toprule
\end{tabular}

%\vspace{-3 mm}
\end{table}


\subsubsection{Experimental Setup}\label{sec:setup}
We conduct all experiments on a Linux server with Intel Xeon 2.40 GHz CPU.
We implement LogSummary with Python 3.6 and make it open-source\footnote{https://github.com/LogSummary/ICSE2021}.
%We adopt Log2Vec\footnote{https://github.com/WeibinMeng/Log2Vec}, which is available to embed words in logs.
% As for MIMICK, we use a popular open-source toolkit\footnote{https://github.com/yuvalpinter/Mimick}. 


\subsection{Evaluation on LogIE}\label{sec:experiment-LogIE}
We intrinsically evaluate the LogIE framework in order to choose its best implementation and compare it to the baselines. We evaluate the main OpenIE methods from the literature as baselines and incorporate them as the OpenIE component of LogIE. For this task, we build and open-source a dataset of log information extraction triples based on public logs. We also use this gold standard dataset to evaluate an improved version of LogIE which uses manually improved templates instead of an online template extraction approach. This serves as an ablation test showing the influence of the template quality on LogIE's performance. 

\subsubsection{Triples Gold Standard Dataset}\label{sec:gt-logie}
\begin{table}[t]
\centering
\renewcommand\tabcolsep{8 pt}
\caption{Resulting number of manually improved templates and manually extracted OpenIE triples from the source datasets for building the OpenIE Gold Standard dataset.}
	\label{table:triples-gt-stats}
\begin{tabular}{ccc}
\toprule
    Source &  Templates &  Triples \\
\midrule
       BGL &       263 &         831 \\
      HDFS &        50 &          87 \\
       HPC &        85 &         199 \\
 Proxifier &        14 &          36 \\
    Switch &        95 &         323 \\
\midrule
    Total &        507 &         1476 \\
\bottomrule
\end{tabular}
\end{table}


This dataset, we employ it as the gold standard for building and evaluating the different approaches within LogIE. The process of building it can be divided into three parts: obtaining the logs data from different services; extracting and improving templates used to assist the triples extraction; and manual annotation. 

We sourced the logs from different types of systems and services. Four of them described in Section \ref{table:summary} are open-source and one of them comes from real world switch logs. 

As part of the process of building the gold propositions dataset we extracted templates from all source logs using LogParse \cite{logparse}.


Then, we manually extracted OpenIE triples from the logs. For each log we manually extracted relational triples of the form ($arg_1$, $r$, $arg_2$), meaning that $arg_1$ is related to $arg_2$ by predicate $r$. We aimed to keep the form (subject, predicate, object) in this order. For this purpose considered both the domain knowledge and the semantic structure. We made several considerations:
We extract (subject, predicate, object) triples in this order.  Where applicable, we make prepositions part of the predicate.
It's required to have at least the predicate and the subject or object present to extract a triple.
We make linking verbs the predicate of a triple where applicable.
Conjunctions, such as “and” or “or”, are split into several triples or combined into a single one where the conjunction is part of the predicate.
For the case of adjuncts, regardless of the kind, we decided to disregard them and simply consider them as separators of two different clauses.
For the cases of apposition, we defined an “is” relation, that would serve as an “is-a” relation which is usually used in ontology building. 

Lastly, we leveraged domain knowledge to extract the values of arguments or attributes as well the instances of different entities. 
Usually these would show up as an “=” or a “:” in the logs. In these cases, we also considered an “is” relation to represent the relation between the two. Additionally, arguments are also represented in the format that command line arguments are written. In these cases, we also use an “is” relation and create a second argument “set” for flags.


\subsubsection{Task Formulation}\label{sec:task-logie} As explained in Section \ref{sec:background}, OpenIE intends to obtain all relations present in a given sentence or corpus together with the arguments or entities related by such relations in a structured manner. Likewise, the goal of LogIE is to extract relations present within each log, which are used as the minimum unit of information from each log. Specifically, given a stream of raw logs as the input, relational triples of the form (arg$_1$, relation, arg$_2$) are to be extracted for each relation present within each log. This task will be tested against the gold standard we propose in Section \ref{sec:gt-logie} and evaluated as detailed in the following Section \ref{sec:metric-logie}.

\subsubsection{Metrics and Baselines}\label{sec:metric-logie}
 The main challenge in order to intrinsically evaluate LogIE—similarly to cases that are common in NLP—is that we need to allow different OpenIE triples extractions to be considered acceptable for the same gold proposition. For this reason, we follow a similar approach to that of Stanovsky et al. \cite{Stanovsky2016oieBenchmark} in their OpenIE benchmark. Inspired by He et al. \cite{HeLuheng2015QuestionAnswerDS}, where the syntactic heads of the predicate and the arguments from a given extraction should match those of the corresponding gold proposition, they define a more lenient approach that considers their token-level overlap instead. Therefore, we use an approach similar to theirs\footnote{https://github.com/gabrielStanovsky/oie-benchmark} to calculate precision and recall of the evaluation. Among the main differences, we do not propagate a match to all matching predicates, but thoroughly test all triples against all gold propositions instead. We don't produce a confidence score for each triple, so we don't calculate AUC scores. The main metric we consider for comparison between the approaches is the F1 score. The metrics are calculated as follows:   
$precision = \frac{\#\ correct\ extractions}{\#\ extractions}$, $recall = \frac{\#\ recalled\ gold\ propositions}{\#\ gold\ propositions}$, $F1 = \frac{2\ \times\ precision\ \times\ recall}{precision\ +\ recall}$.

We compare LogIE with six Open Information Extraction methods, namely, ClausIE \cite{Corro2013ClausIECO}, Ollie \cite{Mausam2012OpenLL}, OpenIE5\footnote{https://github.com/dair-iitd/OpenIE-standalone}, PredPatt \cite{Stanovsky2016GettingMO}, PropS \cite{Stanovsky2016GettingMO} and Stanford OpenIE \cite{Angeli2015LeveragingLS}.

% \subsubsection{Baselines}\label{sec:baselines-logie}
% In the following, we list and introduce the different OpenIE methods that we employ as baselines and also consider within LogIE as its OpenIE component.

% \textbf{ClausIE} \cite{Corro2013ClausIECO} is a clause-based OpenIE approach for the English language. Based on dependency parsing of each sentence, it uses domain knowledge about grammar to identify clauses and their type. Then it performs open relation extraction generating propositions of arguments related between each other in a form that is flexible to obtain OpenIE triples. 

% \textbf{Ollie} \cite{Mausam2012OpenLL} is both a learning-based OpenIE approach and it’s able to consider inter-proposition relationships \cite{Niklaus2018ASO}. It builds on seed triples generated by ReVerb \cite{ReVerbFader2011IdentifyingRF} to learn patterns that may encode various different types of relations. Among these, syntactic, semantic and lexical patterns are learned bootstrapped on the triples from ReVerb and then it uses a matching component to extract them from given sentences.

% \textbf{OpenIE5}\footnote{https://github.com/dair-iitd/OpenIE-standalone} is actually a combination of different OpenIE components itself. Similarly to Ollie \cite{Mausam2012OpenLL}, it is a system able to capture inter-proposition relationships. It builds on CALMIE \cite{CALMIESaha2018OpenIE} which handles conjunctive sentences; BONIE \cite{BONIESaha2017BootstrappingFN}, which deals with numerical sentences; RelNoun \cite{RelNounPal2016DemonymsAC}, which extracts relations mediated by nouns; and SRLIE \cite{SRLIEChristensen2011AnAO}, which extracts triples based on Semantic Role Labeling. 

% \textbf{PredPatt} \cite{predpatt:EMNLP2016} is a framework that serves as a rule- or pattern-based OpenIE approach. They built a layer of semantic pattern annotations on top of the Universal Dependencies (UD) project \cite{Nivre2016UniversalDV}. UD is a framework for consistent grammar annotation across human natural languages. 

% \textbf{PropS} \cite{Stanovsky2016GettingMO} is a rule-based approach for OpenIE. They proposed a different approach going beyond syntax to perform Open Information Extraction. They make a case that some pieces of information cannot be extracted from dependency trees as it’s normally used by the other methods. In contrast, they design a different output representation from semantic trees that enables them to obtain more kinds of propositions. 

% \textbf{Stanford OpenIE} \cite{Angeli2015LeveragingLS} is a clause-based system. They take a clause-based approach by teaching a classifier to define when a clause is to be extracted from a sentence. 


\subsubsection{Experimental Results}\label{sec:eval-public-logie}
We evaluate LogIE and compare it against its manually augmented version and the six OpenIE baselines in Table \ref{table:logie} on the four public logs described in Table \ref{tab:datasets}. 
LogIE learns online templates generated by LogParse \cite{logparse}. However, in order to  perform an ablation test, we also compare LogIE Improved which is an augmented version using manually improved templates that were produced as part of the gold standard dataset introduced in Section \ref{sec:gt-logie}. Then each of the baselines are plain OpenIE approaches used directly on the raw logs. LogIE consistently produces better results across all public logs when compared to the baselines. This is because the pipeline approach of LogIE is optimized to make the most of both the structure and the free text present in logs. On the other hand, plain OpenIE methods are actually meant to be used directly on free natural language text. As you will see in Table \ref{table:logie}, even though both versions of LogIE are consistently superior than the baselines, there are cases where their results could be comparable such as on BGL or HPC. The more free text is present in the logs, the easier it is for plain OpenIE methods to generate correct OpenIE triples. However, as we show in Table \ref{table:logie-speed} applying plain OpenIE methods on the logs is not efficient when compared to LogIE which leverages the templates used as input and the high speed of template matching using tries to produce the OpenIE triples output from the raw logs. The throughput of LogIE is over 200X that of applying plain OpenIE. Nonetheless, the performance of LogIE is sensitive to the accuracy of the templates used as input as shown in the ablation test comparison. As demonstrated by the performance of LogIE Improved, the more accurate templates are, the better the performance of LogIE. Further, LogIE leverages either the structure of the log or the semantic information of the unstructured text within logs to extract information. If there is no rich information in the structure, or if details within the log are omitted to make it shorter, its performance is also affected. This is the case for the HDFS logs where the structured parts don't provide rich information and the natural language implicitly refers to the arguments, which is not picked up by LogIE. This affects its results with a low recall as seen in Table \ref{table:logie}. In turn, this affects the output of LogSummary given the pipeline nature of the framework.
\ 
\smallskip

\begin{table}[t]
\centering
% \renewcommand\tabcolsep{6 pt}
\caption{Test accuracy on the log OpenIE triples gold reference dataset of public logs.}
	\label{table:logie}
\begin{tabular}{ccccc}
\toprule
               Logs &                   Method &       Precision &          Recall &              F1 \\
\midrule
       \multirow{7}*{BGL} &  \textbf{LogIE} &  \textbf{0.918} &  \textbf{0.864} &   \textbf{0.89} \\
                    % &             LogIE &           0.843 &           0.859 &           0.851 \\
                    &                  OpenIE5 &           0.788 &           0.733 &           0.760 \\
                    &                 Stanford &           0.685 &           0.753 &           0.717 \\
                    &                    Ollie &           0.552 &           0.633 &           0.590 \\
                    &                 PredPatt &           0.463 &           0.638 &           0.536 \\
                    &                  ClausIE &           0.447 &           0.602 &           0.513 \\
                    &                    PropS &           0.000 &           0.000 &           0.000 \\
      \multirow{7}*{HDFS} &  \textbf{LogIE} &   \textbf{0.98} &  \textbf{0.459} &  \textbf{0.626} \\
                    % &             LogIE &           0.687 &           0.380 &           0.489 \\
                    &                  ClausIE &           0.159 &           0.530 &           0.244 \\
                    &                  OpenIE5 &           0.271 &           0.220 &           0.243 \\
                    &                 Stanford &           0.184 &           0.210 &           0.196 \\
                    &                 PredPatt &           0.171 &           0.177 &           0.174 \\
                    &                    Ollie &           0.003 &           0.079 &           0.006 \\
                    &                    PropS &           0.000 &           0.000 &           0.000 \\
      \multirow{7}*{HPC} &  \textbf{LogIE} &  \textbf{0.859} &  \textbf{0.667} &  \textbf{0.751} \\
                    % &             LogIE &           0.826 &           0.667 &           0.738 \\
                    &                  ClausIE &           0.588 &           0.648 &           0.616 \\
                    &                 PredPatt &           0.591 &           0.556 &           0.573 \\
                    &                 Stanford &           0.691 &           0.349 &           0.464 \\
                    &                    Ollie &           0.290 &           0.285 &           0.287 \\
                    &                  OpenIE5 &           0.567 &           0.123 &           0.202 \\
                    &                    PropS &           0.000 &           0.000 &           0.000 \\
      \multirow{7}*{Proxifier} &  \textbf{LogIE} &  \textbf{0.869} &  \textbf{0.812} &  \textbf{0.839} \\
                    % &             LogIE &           0.982 &           0.471 &           0.637 \\
                    &                 Stanford &           0.831 &           0.254 &           0.389 \\
                    &                  ClausIE &           0.247 &           0.719 &           0.368 \\
                    &                  OpenIE5 &           0.759 &           0.204 &           0.322 \\
                    &                    Ollie &           0.556 &           0.194 &           0.288 \\
                    &                 PredPatt &           0.061 &           0.106 &           0.078 \\
                    &                    PropS &           0.000 &           0.000 &           0.000 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[t]
\centering
\renewcommand\tabcolsep{18 pt}
\caption{Comparison of speed measured in logs per second between LogIE and the plain OpenIE methods when processing the input logs measured over thirty runs for each OpenIE method and each logs dataset.}
	\label{table:logie-speed}
\begin{tabular}{ccc}
\toprule
\textbf{Approach} & \multicolumn{2}{l}{\textbf{Throughput (logs / s)}} \\
\cmidrule{2-3}
{} &     mean &      std \\
\midrule
LogIE    & 8550.66 & 1909.62 \\
\midrule
OpenIE Methods &   39.05 &   36.19 \\
\bottomrule
\end{tabular}
\end{table}




% \begin{table}[t]
% \centering
% \renewcommand\tabcolsep{5 pt}
% \caption{Test accuracy on the log OpenIE triples gold reference dataset of the case study on real-world logs.}
% 	\label{table:logie-switchlogs}
% \begin{tabular}{ccccc}
% \toprule
%               Logs &                   Method &     Precision &          Recall &              F1 \\
% \midrule
%                   &  \textbf{LogIE Improved} &  \textbf{1.000} &  \textbf{0.711} &  \textbf{0.831} \\
%                   &             LogIE &         0.727 &           0.729 &           0.728 \\
%                   &                 Stanford &         0.783 &           0.668 &           0.721 \\
% Real-world &                  OpenIE5 &         0.548 &           0.578 &           0.563 \\
%  Switch Logs &                    Ollie &         0.526 &           0.385 &           0.445 \\
%                   &                  ClausIE &         0.312 &           0.655 &           0.422 \\
%                   &                 PredPatt &         0.538 &           0.244 &           0.336 \\
%                   &                    PropS &         0.000 &           0.000 &           0.000 \\
% \bottomrule
% \end{tabular}
% \end{table}


\subsection{Evaluation on Ranking Summaries}\label{sec:experiment-summary}
% In this section, we first evaluate LogSummary on four datasets. Then, we introduce a case study to show the usability of LogSummary.

\subsubsection{Metrics and Baselines}\label{sec:metric-summary}
To automatically evaluate the log summarization performance of different approaches, we use ROUGE~\cite{rouge}. The ROUGE metric measures the summary quality by counting the overlapping units between the generated summary and reference summaries. In our scenario, different operators may manually generate summaries in different order of words/phrases. Therefore, we apply ROUGE-1 to evaluate performance.
%%A machine-generated summary (system summary) 
%%reference summaries (typically humanproduced).
Following the common practice~\cite{rouge2}, we report the precision, recall, F1 score for ROUGE-1, where $precision = \frac{\#\ overlapping\ words}{\#\ words\ in \ gold reference}$, $recall = \frac{\#\ overlapping\ words}{\#\ words\ in \ automatic \ summary}$ and $F1 socre = \frac{2 \times precision \times recall}{precision + recall}$  We obtain the metrics using open-source package\footnote{https://github.com/pltrdy/rouge}.
%
We apply the compression ratio, \textit{i.e.,} $\frac{size~of~summaries}{size~of~original~logs}$, to evaluate the log compression performance.
We compare LogSummary with three extractive summarization methods, namely, TF-IDF~\cite{tf-idf}, LDA~\cite{ton19}, TextRank (sentence summary)~\cite{textrank}). %The parameters of these methods are all set best for accuracy. 


\subsubsection{Experimental Results}\label{sec:public-summary}
We compare LogSummary with three baselines on four public datasets.
For LogSummary, we choose top-5 semantic triples from online logs.
Table~\ref{table:summary} show the comparison results of \name{} and three baselins. Overall, \name{} achieves the best summarization accuracy among the four methods.%, \textit{e.g.,} \name{} has an F1 score of 0.864 on Proxifier dataset.
Both TF-IDF and LDA, however, have low F1 scores ($< 0.5$) on all four datasets, because TF-IDF and LDA generate summaries by extracting keywords, which dismisses valuable information in raw logs.
Although TextRank achieves relatively high precision (\textit{e.g.}, 0.904 on the BGL dataset), the high precision is at the cost of low recalls. For instance, on the Proxifier dataset, the recall of TextRank is only 0.050. Because there are many similar logs with different variables, when employed on its own, TextRank may choose many logs of the same type and ignore other types of logs. 
On the contrary, LogSummary, uses LogIE to extract triples from logs as an intermediate representation, which is more fine grained than each complete log, before applying TextRank achieving a $\approx$4.6 times higher recall.
%That is because triples are the smallest semantic units in logs and they are suitable to generate summaries.

% After comparing the readable summaries, we evaluate the compression ratio for summaries. Table~\ref{table:summary} shows the compression ratios (CR) of log summarization on four datasets. We find that LogSummary achieves average compression ratio of 3.1\%, which will vastly reduce the reading load of operators.
In Table~\ref{table:summary} ,we evaluate the compression ratio for log summarization on four datasets. We find that LogSummary achieves average compression ratio of 3.1\%, which will vastly reduce the reading and understanding load of operators.

The results mean that the outputs of LogSummary are not only readable but also highly compressed.
\begin{table}
\centering
% \small
% \renewcommand\tabcolsep{4.5 pt} % 调整表格列间的宽度
\caption{Log summarization performance and Compression Ratio (CR) of LogSummary compared to its Baselines.}
	\label{table:summary}
\begin{tabular}{cccccc}
\toprule
             Logs &      Method& Precision & Recall & F1 & CR  \\
\midrule

                  
\multirow{4}*{BGL}&  \textbf{LogSummary} &\textbf{0.815} &\textbf{0.703} &\textbf{0.725} &\textbf{0.026} \\
                  &   LDA      &   0.382   &  0.076 &   0.119 & 0.130\\
                  & TextRank   &   0.893   &  0.238 &   0.347 & 0.144\\
                  & TF-IDF    &   0.383   &  0.354 &   0.332 & 0.024 \\
                  
\multirow{4}*{HDFS}&  \textbf{LogSummary} & \textbf{0.759} &\textbf{0.432}& \textbf{0.538} & \textbf{0.015}\\
                  &   LDA      &   0.220   &  0.045 &   0.074 & 0.225\\
                  & TextRank   &   0.602   &  0.079 &   0.135 & 0.230\\
                  & TF-IDF    &   0.193   &  0.176 &   0.179 & 0.033 \\

\multirow{4}*{HPC}&  \textbf{LogSummary}&\textbf{0.819}&\textbf{0.911}&\textbf{0.840} &\textbf{0.037}\\
                  &   LDA      &   0.530   &  0.110 &   0.175 & 0.251 \\
                  & TextRank   &   0.904   &  0.265 &   0.365 & 0.208\\
                  &  TF-IDF    &   0.487   &  0.506 &   0.472 & 0.039 \\
 
\multirow{4}*{Proxifier}&   \textbf{LogSummary} &\textbf{0.879}&\textbf{0.857} &\textbf{0.864} &\textbf{0.045}\\
                  &   LDA      &   0.332   &  0.088 &   0.135 & 0.099\\
                  & TextRank   &   0.663   &  0.050 &   0.093 & 0.275\\
                  & TF-IDF&   0.281   &  0.324 &   0.290 & 0.023\\
                  
\bottomrule
\end{tabular}
\end{table}





\begin{figure}
      \begin{minipage}[h]{1.0\linewidth}
      \centering
      \includegraphics[width = 8.5 cm]{figures/case-study-logs.pdf}\\
      \end{minipage}
      \vspace{-1 mm}
       \caption{A case study of LogSummary on switch logs.}\label{fig:case-study-logs}
    % \vspace{-2 mm} 
\end{figure} 



\subsection{Threats to Validility}
The LogSummary framework leverages each of its components to automatically produce accurate summaries. 
However, its pipeline nature makes each component dependant on the quality of the output from the previous ones. 
Sometimes, we should proceed to improve the templates manually since template extraction is not perfectly precise. 
These imprecisions meant there would be redundant templates extracted from the logs. Additionally, in some cases, the variables may not have been detected properly.
Therefore, the quality of the templates may affect the triples extracted by LogIE, which in turn affects the representations built by Log2Vec \cite{log2vec} which are used by TextRank \cite{textrank} to produce the ranked summaries. 
Nonetheless, each of the components provides significant benefits over their baselines. 
LogIE produces triples at over 200 times the throughput of plain OpenIE methods, which serve as the intermediate result that LogSummary leverages to achieve $\approx$4.6 times the recall of TextRank \cite{textrank}, which is the best performing baseline.
LogSummary can serve further downstream purposes, which we consider for future work. 
The triples of LogSummary could aid the creation of knowledge graphs applied to perform automatic root cause analysis. Additionally they could serve as the intermediate representation before other log analysis tasks.
LogSummary could produce the summary of anomalous logs for troubleshooting.
Further, we consider five log datasets as part of the evaluation from online system services. Our approaches outperform their baselines in all of them, which shows the generalizability of LogSummary. However, it may encounter challenges when dealing with complex application layer logs, \textit{e.g.,} operators create complex rules for the Rule Extraction part.

==> arXiv_ICSE SEIP/intro.tex <==
%系统越来越复杂，service management越来越重要
With the continuous development of Internet applications, large-scale online software service systems (\textit{services} for short hereinafter) are getting increasingly large and complex.
A non-trivial service anomaly can impact the user experience of millions of users and lead to significant revenue loss~\cite{pi2019semantic}.
Consequently, the reliability of online services is of vital importance.

%很多大型服务会用日志来做运维
Large-scale services usually generate logs (see the top half of Fig.~\ref{fig:logs}), which describe a vast range of events observed by them and are often the only available data recording service runtime information.
% Therefore, logs are crucial for service management~\cite{deeplog}.
%%目前有了很多基于日志的自动化运维工具，然而他们还需要人工的去分析根因
Therefore, many automatic log analysis approaches have been proposed for service management~\cite{he2020survey}, which can be classified into log compression methods (\eg \cite{logzip}), log parsing methods (\eg \cite{logparse,zhu2019tools}), anomaly detection methods (\eg \cite{deeplog,loganomaly}), failure prediction methods (\eg\cite{zhang2018prefix}), failure diagnosis methods (\eg \cite{zhou2019latent}), \emph{etc.}
Although these approaches help operators efficiently understand the status of services, they leave the burden of summarizing logs to operators.
% have beed designed for monitoring status \cite{Khatuya2018ADELEAD,he2018identifying}, anomaly detection \cite{deeplog,zhang2018prefix,loganomaly}.
% However, even though monitoring status approaches help operators understand the target service more efficiently, they leave the burden of status analysis to operators. %For example, they only show some structured data to show the status of services. They still require operators to have domain knowledge. 
%%削弱异常检测
%Anomaly detection approaches report potential problems~\cite{pi2019semantic} and generate alarms for anomalies~\cite{zhang2018prefix}, which reduce the time to discover anomalies. 
%Despite advances in anomaly detection approaches, troubleshooting today still remains largely manual.
More specifically, after a failure is detected/predicted/diagnosed, operators still have to read the corresponding original logs (\ie a log sequence) to make sense of service-wide semantics~\cite{dogga2019system}.
% it still entails reading the original logs and understanding the context manually by the operators, in order to find events, troubleshoot or identify the root cause. 
This is because the existing automatic log analysis approaches, especially those for failure prediction or diagnosis purpose, are not that accurate and general for every scenario. 
Operators must make sure a failure has occurred or will occur before they take measures to mitigate or avoid failures.
% Operators are still responsible for making sense of service-wide semantics, bridging together outputs and features from existing analysis tools~\cite{dogga2019system}. 
%It entails reading the original logs and understanding the context manually by the operators, in order to troubleshoot and identify the root cause. This is because operators are still responsible for making sense of service-wide semantics, bridging together outputs and features from existing analysis tools~\cite{dogga2019system}. Their expertise is key to sort through the boilerplate and the noise of normal logs and unimportant data so as to understand the log stream. 
 
%%但人工分析日志非常麻烦, 所以工程师需要一个自动准确的日志摘要方法
However, manual log summarization, or the rule (\eg regular expression rule) based log summarization, has become ineffective and inefficient because of the following three reasons.
(1) A large-scale service is usually implemented and maintained by hundreds of developers and operators. 
The developers or operators who investigate logs often have incomplete knowledge of the original logging purpose.
(2) 
%Usually, a developer or operator has incomplete knowledge of the overall service, and none of them is familiar with all logs generated by services. 
The volume of logs is proliferating, for instance, at a rate of about 50 gigabytes (around 120$ \sim $200 million lines) per hour~\cite{zhu2019tools}.
The traditional way of log summarization which largely relies on manual inspection or rule-update has become a labor-intensive and error-prone task.
(3) With agile software development becoming increasingly more popular, operators deploy software updates more frequently, leading to a large number of new types of logs being generated continuously.
It is very difficult for operators to timely comprehend these new types of logs.
Although several works have been proposed for log compression~\cite{gentili2012data, logzip} or system interpretability through logs~\cite{jianguanglou2010mining, ton19}, to the best of our knowledge, there is no previous work aiming to help operators efficiently and effectively summarize a given log sequence in an interpretable and readable manner.
% facilitate the interpretability and readability of the logs for the operators to quickly comprehend the system behaviour.
% \textcolor{red}{Detailed logging is generally avoided in production environments because it can generate too much log data and, at high frequencies, perturb the system. However, log data can be essential for understanding interactions in a complex system.}
%
% There has been previous research on log compression \cite{gentili2012data} or system interpretability through logs \cite{jianguanglou2010mining, ton19}, but none of them aiming to facilitate the interpretability and readability of the logs for the operators to quickly comprehend the system behaviour.

%\vspace{2 mm}
\begin{figure}
      \begin{minipage}{1.0\linewidth}
      \centering
      \includegraphics[width = 8.5 cm]{./figures/logs.pdf}\\
      \end{minipage}
%      \vspace{-2 mm}
       \caption{Log stream example and summaries.}\label{fig:logs}
    %   \vspace{-1 mm}
\end{figure} 


%keywords不合适
 %Obtaining keywords, which is the typical approach to summarize text, is inaccurate in our scenario~\cite{potharaju2013juggling}. They only consider the presence of a keyword regardless of where it appears and its relationship to other words (e.g., ``loss'' in ``packet is not loss''). In our case, we require to keep the semantics present in the logs for the output summary to be readable. 

%like jigsaw
% \textcolor{red}{
When operators investigate logs, they usually care about three key pieces of information, \textit{i.e., } ``entities'',  ``events'' and the ``relation'' between them.
% These information will help operators to check running status and quickly locate problems. 
% introduce triple extraction
% To address this, we extract relational triples from logs containing this information in its summarized form. 
In Fig. \ref{fig:logs}, for example, (``Interface'', ``changed to '', ``down'') is the expected relational triples  extracted from the first log.
These triples are easy to understand for operators because they keep both the semantics and syntax of the original log~\cite{ApplicationsMausam2016OpenIE}.
If we can automatically provide operators the \emph{summarized triples} of the \emph{important} logs in a given log sequence, operators can gain a clear view of this log sequence.
% Therefore, we try to summarize logs for online services and rank them by informativeness.
The original goal of service logs, \ie ``\textit{logs are designed for operators to read}'', motivates us to apply natural language processing (NLP) methods to summarize logs.
% }
% 
% Obtaining keywords is a typical approach to summarize logs. 
% However, keyword summaries are not going to provide above information.
% Keywords consider the presence of a keyword regardless of where it appears and its relationship to other words (e.g., ``loss'' in ``packet is not loss'').
% It is inaccurate in our scenario~\cite{potharaju2013juggling}, since we require to keep the semantics present in the logs for the output summary to be readable.
% Relations of words (e.g., entities, actions) are lost if only keywords are used for summarization.
% Automatically summarizing logs, \ie extracting valuable information from logs, not only provides operators a clear view of services, but also reduces operators' efforts for manual analysis. 
% Therefore, operators need an automatic and accurate summarization approach for log analysis and further troubleshooting.
A large number of works have been proposed for text summarization in NLP domain~\cite{jipeng2019short}.
However, there are four following challenges lying in applying existing NLP methods for log summarization.
% It is inaccurate in our scenario~\cite{potharaju2013juggling}, since we require to keep the semantics present in the logs for the output summary to be readable. Extracting valuable information automatically from logs not only provides operators a clear view of services, but also reduces the operators' efforts for manual analysis. Therefore, operators need an automatic and accurate summarization approach for log analysis and further troubleshooting.
% However, there are several challenges to develop log summarization as follows.
%4个挑战
\begin{enumerate}
\item It is difficult for the existing NLP tools to accurately extract the expected triples from logs,
% extract valuable information from logs. 
because logs not only contain normal words, but also domain-specific symbols, and the syntax of a large portion of logs significantly differs from normal sentences.
% are not only formed by natural language absolutely, they contain many domain-specific symbols and grammar.

\item 
Online services can generate a huge number of logs in a short period.
Typically, operators usually investigate all the logs of some period (say one hour before a failure) to obtain the summary of these logs~\cite{gunter2007log}.
Applying existing NLP tools to extract triples for each newly generated log is computationally inefficient (see Table~\ref{table:logie-speed}). 


\item  
Existing NLP methods usually summarize texts based on the order of sentences (logs) \cite{kryscinski2019neural}. 
However, for a given log sequence, operators expect to read the summarization of \emph{important} logs first.
Therefore, there is a huge gap between the expectation of operators and the summarization generated by existing NLP methods.
% Logs are generated in the order of program executing, NLP summarization tools also generate summaries based on the order of original text, which conflict with the expectations of operators. Operators prefer to choose and read important events first.%, however traditional methods cannot rank summaries based domain-specific meaning.

\item 
% LP summarization tools has been studied with natural language datasets of large, paired document-summary examples. 
% However, such log datasets are rare and the models trained from them do not generalize to logs. 
% For real-world services, there exist only raw logs and no reference summaries.
Applying NLP methods to learn a text summarization model usually needs a large-scale training set~\cite{jipeng2019short}.
However, to the best of our knowledge, although there are publicly available log datasets~\cite{zhu2019tools}, there is no publicly available dataset for log summarization yet.



\end{enumerate}



%介绍LogSummary
To address the above challenges, we propose LogSummary, an automatic, unsupervised end-to-end log summarization framework for online services. 
The goal of LogSummary is to obtain the summarized triples of important logs for a given log sequence, which takes both semantic information and domain knowledge into consideration.
% Similar to \cite{gunter2007log},  we focus on summarizing logs over a user-provided time period.
% LogSummary accurately summarizes important information and gets rid of the noise for any log sequence.
% Specifically, developers design formats of logs to be ``printf''-ed by services~\cite{hpdc19} so they can be read for troubleshooting.
% In this work, we consider the setting where there are logs with no summaries provided.
% , and propose an end-to-end architecture to perform unsupervised log summarization.
The contributions of this paper are summarized as follows.

%contributions   
\begin{enumerate}

\item We propose LogSummary, a framework to perform log summarization for online services.
For a given log sequence, LogSummary obtains the summarized triples of important logs. 
The summary preserves the important information of this log sequence, and is easy to understand.
% which reduce the amount of log messages generated by several orders of magnitude, while still easy to understand and preserving their key information.
The implementation of LogSummary is available online\footnote{https://github.com/LogSummary/ICSE2021}.
%LogSummary
% \item \textcolor{blue}{LogSummary, the first work to perform automatic summarization of real-time logs, which generates highly compressed (average compression ratio of 3.1\%) and readable summaries (average ROUGE F1 score of 0.741) of the target log streams. The whole implementation of LogSummary is available online\footnote{To preserve anonymity, we uploaded the code as attachments.}}.


\item We propose LogIE (Log Information Extraction), a domain-specific and efficient information extraction approach. 
It accurately extracts the expected triples for each log by integrating it with domain knowledge (addressing challenge 1), and achieving efficient information extraction by combining it with log template (addressing challenge 2).
% The output of LogIE are relational triples, the most fine-grained semantic elements in logs, which are summaries of logs. 

\item 
% We design a mechanism to rank summaries based on their importance and help operators to read/understand logs faster. 
% To the best of our knowledge, this is the first work on ranking log summaries.
We propose a simple yet effective method to rank the triples generated by LogIE.
It ranks triples according to the global knowledge learned from all logs, rather than the local information of each triple.
In this way, LogSummary accurately obtains the triples of \emph{important} logs expected by operators (addressing challenge 3).

\item Given the lack of a publicly-available gold standard for log summarization, we manually labelled reference summaries for four existing open-source log datasets and make them available on github\footnote{https://github.com/LogSummary/ICSE2021/tree/main/data}.  We believe that the availability of a summary gold standard would benefit future research and facilitate the adoption of automated log summarization.
\end{enumerate}


The rest of the paper is organized as follows: 
We discuss background in Section \ref{sec:background}, highlight the challenges in Section \ref{sec:challenge} and propose our approach in Section \ref{sec:design}. 
The evaluation is shown in Section \ref{sec:evaluation}.
In Section \ref{sec:related}, we introduce the related works. 
% In Section \ref{sec:discussion}, we discuss the practicability of LogSummary.
Lastly, we conclude our work in Section \ref{sec:conclusion}.



==> arXiv_ICSE SEIP/related_work.tex <==

% Traditional information extraction approaches rely on predefining a limited set of target relations and hand-crafted patterns. For this they would adapt Named Entity Recognizers and dependency parsers to target a specific domain. These approaches would then require manual effort to be repurposed and applied to a different domain. In order to address the challenge of scalability for performing web information extraction, Banko \textit{et al}. \cite{Banko2008OpenIE} introduced Open Information Extraction (OpenIE). They presented a new information extraction paradigm that would allow to extract relations without defining the number or type of relations in advance. 

Different kinds of log summarization approaches have been proposed for purposes different from ours. 
At the same time, different methods have been used for similar purposes as to enhance the interpretability of the logs for troubleshooting. 

Gentili \textit{et al.} \cite{gentili2012data} proposed an approach to leverage a taxonomy graph over the events presented by the logs in order to reduce the resulting raw data size to keep the required space to store the data manageable and improve the performance and system load for log analysis. 
Gunter \textit{et al.} \cite{gunter2007log} presented an approach for log summarization for the goal of decreasing the load on the system for logging. They do not focus on human interpretability of the logs, but rather on reducing system workload for downstream tasks. Their main evaluation metric is keeping the same performance of autonomous anomaly detection despite the compressed logs.
Shang and Syer focus on understanding software logs \cite{shang2014understanding} and examining the stability of logs \cite{kabinna2018examining}.
He \textit{et al.} \cite{he2018identifying} presented a method to identify impactful service problems by using log analysis. They pay more attention to visualization rather than readable.


% Since then, various different OIE methods have been proposed taking different approaches. Niklaus \textit{et al}. \cite{Niklaus2018ASO} categorized them into four categories.
% Rule-based, where a predefined set of rules over the grammar structure allows for automatically finding OIE triples such as PredPatt \cite{predpatt:EMNLP2016} or PropS \cite{Stanovsky2016GettingMO}. These rules are generally based out of the dependency tree which can be very accurately built out of sentences.
% Learning-based approaches which may be bootstrapped with rule-based methods to generate training data to be used for training like Ollie \cite{Mausam2012OpenLL} with ReVerb \cite{ReVerbFader2011IdentifyingRF}.
% Clause-based approaches that make use of grammar rules to decompose the sentence into smaller and syntactically simplified ones, where each of them are themselves clauses, in order to extract more relations such as Stanford OpenIE \cite{Angeli2015LeveragingLS} or ClauseIE \cite{Corro2013ClausIECO}. 
% Approaches that consider inter-proposition relationships, including hypothetical cases and conditionals. An example of this is OpenIE5 which is a system composed of different OIE components dealing with subtasks of OIE \cite{CALMIESaha2018OpenIE,BONIESaha2017BootstrappingFN,RelNounPal2016DemonymsAC,SRLIEChristensen2011AnAO}.

% DeepLog \cite{deeplog} combines workflow discovery approach together with anomaly detection to facilitate root cause analysis, so once an anomaly is detected it can be associated with a workflow \cite{jianguanglou2010mining}. However these workflows may not be as low-level as needed to show the underlying complex workflows where the problem happened. A similar case is \cite{li2017flap}, where they propose an event summarization approach similar to \cite{jianguanglou2010mining} as part of their comprehensive log analysis platform. In contrast, our proposed summarization approach is more flexible as an operator could arbitrarily select any given sequence of logs of an arbitrary size and produce a summary.


% Lots of previous work in NLP domain focuses on text summarization generates summaries from input documents while keeping salient information. It is an important task in NLP domain and can be applied to several real-world applications. 
% There are two main text summarization techniques: extractive and abstractive. Extractive summarization generates summary by selecting salient sentences or phrases from the source text, while abstractive methods paraphrase and restructure sentences to compose the summary. Many popular extractive summarization techniques do not require example summaries and instead consider summarization as a sentence-selection (e.g, TextRank\cite{textrank}) or keyword-selection (e.g, LDA\cite{Ramage2009Labeled}) problem. Sentences may be selected based on scores computed from the presence of topic-words or word-frequencies \cite{nenkova2005impact}. Gaetano Rossiello \textit{et al.}~\cite{rossiello2017centroid} extends this approach by mapping sentences to their representation using word2vec embeddings rather than using TF-IDF weights. While abstractive summarization involves paraphrasing the context-aware sentences after understanding the language \cite{paulus2017deep,nallapati2016abstractive}. Abstractive techniques generally requires large-scale data (documents and corresponding summaries) for training the models, for example news titles can be considered as summaries and the articles can be considered as the document. However, logs do not have the corresponding summaries for training.


% The aforementioned works deal with properly written regular text and are not directly applicable to our domain. In contrast, LogSummary focuses on logs to extract domain-sepcific information and perform log summarization.
% Short-text summarization or compression has been tackled in the NLP field facing similar challenges to the ones we face with logs. Logs are pieces of short text that come in a temporal stream of data, which can also be found in other scenarios. In the field of NLP, short text analysis and mining has become more and more important with the advent of social media. Specifically for cases such as Twitter or Sina Weibo, which are an analogous scenario where a constant stream of short texts are generated.
% Short texts present different challenges from documents text corpus. Their representation becomes more challenging given the sparsity that it imposes if the usual bag of words and weighted representations are used. Additionally, there is less syntactic information to learn from if texts are short. 
% Common approaches such as latent Dirichlet allocation (LDA) \cite{Blei2003Latent} do not perform well on short text because of its inherent short length and therefore its sparseness. Considering such challenge, \cite{jipeng2019shorttext:survey} presents a survey on short text topic modeling techniques applications and performance. They divide these methods into three categories depending on their approach, these being Dirichlet multinomial mixture, global word co-occurrences, and self-aggregation. Particularly, the self-aggregation approach solves the sparseness problem in short texts by combining short texts into longer ones as pseudo-documents before applying topic modeling. LogSummary, takes an approach similar to self-aggregation, while using more fine-grained semantic pieces obtained from LogIE from each of the logs within the target log stream.

Satpathi \textit{et al.} \cite{ton19} proposed the first closely related work in our scenario. Their focus is different from ours as they aim to mine the distribution of messages for each anomalous event and their occurrences in the logs getting an event signature that represents it formed by keywords. Nonetheless, they use an approach that resembles log summarization by first aggregating all the events from the given distribution using their proposed change-point detection and then performing summarization using LDA \cite{Blei2003Latent}. However, LDA has proven not to work properly for short text summarization despite aggregation or previous clustering. Additionally, they do not consider parameters from the logs that are key to understanding an event after summarization and helping operators with their troubleshooting. 


% \textbf{ClausIE} \cite{Corro2013ClausIECO} is a clause-based OpenIE approach for the English language. Based on dependency parsing of each sentence, it uses domain knowledge about grammar to identify clauses and their type. Then it performs open relation extraction generating propositions of arguments related between each other in a form that is flexible to obtain OpenIE triples. 

% \textbf{Ollie} \cite{Mausam2012OpenLL} is both a learning-based OpenIE approach and it’s able to consider inter-proposition relationships \cite{Niklaus2018ASO}. It builds on seed triples generated by ReVerb \cite{ReVerbFader2011IdentifyingRF} to learn patterns that may encode various different types of relations. Among these, syntactic, semantic and lexical patterns are learned bootstrapped on the triples from ReVerb and then it uses a matching component to extract them from given sentences.

% \textbf{OpenIE5}\footnote{https://github.com/dair-iitd/OpenIE-standalone} is actually a combination of different OpenIE components itself. Similarly to Ollie \cite{Mausam2012OpenLL}, it is a system able to capture inter-proposition relationships. It builds on CALMIE \cite{CALMIESaha2018OpenIE} which handles conjunctive sentences; BONIE \cite{BONIESaha2017BootstrappingFN}, which deals with numerical sentences; RelNoun \cite{RelNounPal2016DemonymsAC}, which extracts relations mediated by nouns; and SRLIE \cite{SRLIEChristensen2011AnAO}, which extracts triples based on Semantic Role Labeling. 

% \textbf{PredPatt} \cite{predpatt:EMNLP2016} is a framework that serves as a rule- or pattern-based OpenIE approach. They built a layer of semantic pattern annotations on top of the Universal Dependencies (UD) project \cite{Nivre2016UniversalDV}. UD is a framework for consistent grammar annotation across human natural languages. 

% \textbf{PropS} \cite{Stanovsky2016GettingMO} is a rule-based approach for OpenIE. They proposed a different approach going beyond syntax to perform Open Information Extraction. They make a case that some pieces of information cannot be extracted from dependency trees as it’s normally used by the other methods. In contrast, they design a different output representation from semantic trees that enables them to obtain more kinds of propositions. 

% \textbf{Stanford OpenIE} \cite{Angeli2015LeveragingLS} is a clause-based system. They take a clause-based approach by teaching a classifier to define when a clause is to be extracted from a sentence. 



==> discussion.tex <==

The LogSummary framework leverages each of its components to automatically produce accurate summaries. However, its pipeline nature makes each component dependant on the quality of the output from the previous ones. Therefore, the quality of the templates may affect the triples extracted by LogIE, which in turn affects the representations built by Log2Vec \cite{log2vec} which are used by TextRank \cite{textrank} to produce the final summary of LogSummary. Nonetheless, each of the components provides significant benefits over their baselines. LogIE produces triples at over 200 times the throughput of plain OpenIE methods, which serve as the intermediate result that LogSummary leverages to achieve $\approx$4.6 times the recall of TextRank \cite{textrank}, which is the best performing baseline.
Both LogSummary and LogIE can serve further downstream purposes, which we consider for future work. The triples output of LogIE could aid the creation of knowledge graphs applied to perform automatic root cause analysis. Additionally they could serve as the intermediate representation before other log analysis tasks. LogSummary could produce the summary of anomalous logs for troubleshooting.
Further, we consider five log datasets as part of the evaluation from online system services. Our approaches outperform their baselines in all of them, which shows the generalizability of LogSummary.


% brainstorming
% We can discuss the subjectivity of the summarization evaluation and how we reduce it with the gold standard

% Analysis: the difference between logIE and OpenIE, and why we run fast. 


% The importance of the quality of the templates given that its a pipeline method for LogIE. Similar points for LogSummary.

% We could explain that we use the gold standard as input and it performs better than the online one but this is a novel approach and we pave the way for future improvement

% Discuss somehow about the novelty of logsummary and its pros/(cons) in its application

%Future works: We could apply LogIE to build knowledge graph for root cause analysis. Structured triples are intermediate representations in other log analysis tasks (\textit{e.g.,} log-based anomaly detection).  We can use LogSummary to do alarm compression.

% One limitation of LogSummary is that it is a pipeline framework, which consists of many modules. If previous modules perform bad, the output of LogSummary may be bad as well. For example, the accuracy of template extraction is essential to LogSummary.



